Language statistics at different spatial, temporal, and grammatical scales

Statistical linguistics has advanced considerably in recent decades as data has become available. This has allowed researchers to study how statistical properties of languages change over time. In this work, we use data from Twitter to explore English and Spanish considering the rank diversity at different scales: temporal (from 3 to 96 hour intervals), spatial (from 3km to 3000+km radii), and grammatical (from monograms to pentagrams). We find that all three scales are relevant. However, the greatest changes come from variations in the grammatical scale. At the lowest grammatical scale (monograms), the rank diversity curves are most similar, independently on the values of other scales, languages, and countries. As the grammatical scale grows, the rank diversity curves vary more depending on the temporal and spatial scales, as well as on the language and country. We also study the statistics of Twitter-specific tokens: emojis, hashtags, and user mentions. These particular type of tokens show a sigmoid kind of behaviour as a rank diversity function. Our results are helpful to quantify aspects of language statistics that seem universal and what may lead to variations.

==> img/fits_pdf/Mexico/displaying_scale/1grams/12hrs <==
%PDF-1.4
%¨‹ ´∫
1 0 obj
<< /Pages 2 0 R /Type /Catalog >>
endobj
8 0 obj
<< /ExtGState 4 0 R /Font 3 0 R /Pattern 5 0 R
/ProcSet [ /PDF /Text /ImageB /ImageC /ImageI ] /Shading 6 0 R
/XObject 7 0 R >>
endobj
10 0 obj
<< /Annots [ ] /Contents 9 0 R
/Group << /CS /DeviceRGB /S /Transparency /Type /Group >>
/MediaBox [ 0 0 720 504 ] /Parent 2 0 R /Resources 8 0 R /Type /Page >>
endobj
9 0 obj
<< /Filter /FlateDecode /Length 11 0 R >>
stream
xú’ù]ìm∑qûÔÁW¨K∫J‹ƒ˜«Ö.D€QU™R)Z,Á"ŒsD”§…¢eYŒøœ˚k/ºç}f»3—D6]Úô›É¡çF£`m|˜‰èow|áˇ˝È¯ü«ˇ¬øø?¸Ò[¸Ôõ'áOﬂ?’¿ﬂè≥K¯È˛Ô?==˝„”gøA—?†ƒoü∫;Jƒ_î‘¯√˚ÒCJÒñ>‡∑◊œ„/:Ê‰‹éÿÛ/_ˇ„¯·¯Ï7ÅuÜ„ø¢h€≠IÎ‹≠tÁ{qµ%<Ù≥ø˘˙ﬂæ}˜ıﬂ˝ˆÛ„›ûºœ∑X¯≥)Ú˘z¯”Ôûæ8~∫?ƒAxTÄﬂºT_Ó∑Ã⁄>áˇÙÙ˛ø;>u®Àªrñôœ≠74’á|º˚˛ÈÛ/©’[Ø%Hæ¸˝”gˇÖq|˘èOü¯ø:æ¸Óâ¢K•’å*Q‰w˛"ÂÊŒ∫‚≠ÖÒ√YE5ÃÇ˚Â”£ã~˝∆‡nMõ⁄∏>ΩJ∑œ‘ı¨^£˜£Ñ√-©=Í’ï‰ﬁBØ˛≠ıöC∫ı–{ISÚ˘U∫}°ægıõa€£L,9¥ˇØvﬁZø=ﬂ≤oÆ◊©éıÒgµ[>†›gk+~jˆm:·®«P„Èå÷ÁWu„Ö˙ﬁ∏#∂Âzˆ˛|˙¸∫é<_ﬂ€v$¯àI‚‹}yêœØÍ»ıΩqGbªïúcª?x}~]GûØÔç;í€-cÏ·aÊÉ◊Á◊u‰˘˙ﬁ∏#5›™œ˝n”Ú˘uyææ7ÓHk∑rjß∑îœØÎ»ÛıΩmG¢s∑Ë|(ßÂÛ´:ÚB}o‹Ônµñt˜2Ú˘uyææ7ÓHÛ∑⁄C©Á‰îœØÎ»ÛıΩmGíØ∑ñcòèΩ>Ω™œ‘ı∆@KSl˘T‹˙¯∫.<W€w¢ƒ[h…µ~>w}~]7ûØÔç;R˚-ıÓÓv,ü_◊ëÁÎ{„éthÃµrÓıÒu›xÆ∂∑ÌDFXÌZJ˜B>ø™/‘˜∆¡1Á~z˘Î”Î:Ò·∫ﬁ∏≠‹rÕ-ûR>øÆœ◊˜∂)!‹FvÈ‹ﬁÀÁWu‰Ö˙ÓŸì1âiÑ%9 ©ópO
º˚Äp†≈‡"7˛35„ôæ˘3i3ÒÕ=ôêŒ\√ß˛f≥:öíI∑îcÒë9ìt@p™À#ÎpÏ5úç˚áOF—xÉ¢c©˛J\H˛y…ºÛ˘j¶÷ÚWoûºpj
Îû^]ü?./¥UE{µuÕÅ˛¸Àcı∞`3›#tSº~sπÖ‹Î‘ımh˚`Áﬂ™ÎñVj)=ù}¡GwﬁT6zok{©˚>Â[´Ωy,Ωü˝oﬁˇ‡˚
:O˘ﬁ|tˇMe£ˇ∂∂ó˙‡§±9…µª‚¸ŸˇÙˆ˝Á˛.π‡Ø˛/¡«˜_+õ˝7µΩÿˇñ‡Gbå=Œ˛ó7ÔÃà‡1Jh¡Ïø>∫ˇ¶≤—[€K˝è9›\»Æ˜V\:˚ﬂﬁºˇ)TÑi±∆{ˇE—˝7ïç˛€⁄^Í
ëk:ä+£ˇ~˘?Û7\!?ÂZYPb.!1¯èâ5}˘˝`k¨·˜ˇ…?œ‰#ïË—vU¢«ÙD€BÕOòïÂ¸Ø‚7X[1á~¸›o´_ZòﬁªÓ∂ƒc∑\ÂÍ Yºé?π$Œ…âız´—±ÒÔ5√‰]¬Çû\•xÂk¥õGuù≈%˝Åf‹b.1sL$õÄ`·ÊkàÅOΩÄ—&ECD€èÒB,GÂëx¬W¥‹D.=ó2äg,a´?J‡Åª3 Àçùß€G£#É*ºıƒ?8|Å˜G˝√q |∏·I-˜√èÕQ-≥95†≥!R•c˘®Ωå˙+¨.2j?|ã"D\‘∞d|«ÃÃÒ\ÿ™èæQi›q@˙l?>ÑÇ"¡é˘ñÍê¶[!W?‰5E7¶wÏÌÊ;»}ÅV#Ú˛)°Pâç>vC--Ö!œ∞´1®ÌÜ'˜ñÜCù@Ë⁄≠πÑSÓÒ0Â˘Üè≠Ly∫µ8∞œò—‡îü…âÄE∏%è†íRl≈zc@˜RôbgáÖ†Ò9‹B*a@Ê0¥°WVéQ¯”:	K@skDß∞Ò∆ƒçC		-∆å¨√£ò\-m °…êc‚πÿ˚x.L'ªÑQ?&›'•Êáºa<6vîÔ*¥ÑÚÑëh•q°¬$Ò–ÎËÎïƒ≥Ê‰g®>¡4á6[∆Jú`çˇq®»óèáRQ’%Ù0bNa.“!œ∞Kü9Ã°”T†©6‰àn}§r8øz ˝!áQò:ã9€cüˆäﬂﬂ2c–!Ô¥úËÜ2¢§k£û Ω∆êrfrƒpœB0Ò!øRh!6EpNc∞
ˆ™)#Ä<8Ø3:Fø
Õës “!’˝q£/CW!gÀú/Ckï™j∂0&ºa8((	mpÜLπsp<clk§óÛgyës@1(1˝}?’ÃP¶wMüPÛ–YÂ_&Nx.a∏3…ÖDå|ÄÌ1LSçÑÿq›ƒ.e»·|Ü˘çı„Äô<‰ëS}Ç<rVúS6∑€`ïn∫(}¥Fc[1Ã¿q$cqÎln,\Í4ò'FæıàPúÉç’.¡‡†€ÇéP¨8
gì‡y:>Aä¿Ç˝0Ç+aB7ïΩ;'Ï≥z¨å(é0’ûFWaàò≈ï]‚⁄2∫1‰ùãâé.∏’`	·, àƒaé∑úºﬁ)”;µÏπs…X–Úê®Â∞yDiàaÚW˙/òjˆa»W⁄≈qÈ@Ã;´«ﬂ∂Nßµ5ŒÆ
*ŸÍi(Ñˆt»#÷/Ãç6‰0Ñ0è|9Ïˆ‰π`*t∫å!¶
]^‚2X tx∫Œ)Ç‚‹8£¡£9úF*ä3gBvê·Z1ãsî∂¯=;c+ß^±<é¬Kuòï`J˚ƒå≥≠≥ØÊÊ(˜úƒuÿ*∫éû÷≠0ºvÑ˚<Î9,´˜Dne‘àÖ´õãmtU˚anïÜ∫`b”›Ú¬Ú^~ùî∞rx8lÓÎáé∞Úé…ê±\`^b≠ŸÎß[km¥û]ÒS%¯ÊüÀ.bËCﬁπÚ´‘aç0-ƒbµ?à·[∞@m⁄¡bÑôú’áÙƒSjŸq†âcmƒXÌŸ°:Zÿ1= Ë)ñ`<Í6œd:£„ü]^/yﬂ7
¿Ÿa=alcç)rR˜VÍ¡¬ÿ#oå,r	q˛¡RSG6Y=ºb ±éfÆ£XÔ6˝BäXÃ
Á°çI˛.$nJÄá_vû Å?ÇáÕ≥<W{Døa3»‰QèëgÆû∞≥%Ê≤ûΩG
æ= ¢è≤Yñu,¡≠¶≠W
∆N€Ÿ
9÷lü˝^
tâpm7æÃTN(Cg:a!Ôy,"õ‹sõsJ´g|Öêª•ÕÊ3˜hïﬂËwf∞Ç0ï“°ÓrZfÈDΩˆπàÛÙq∂<ïå≈ølÉòô(,.Ô~+ÀÏ√Âöz∆*ò¸ÆNnTZa¸k—çGÄ(∆˙(»—‚B7j cqEç√ΩSÜ°¿ò†¶øàí2úQÿMø†3à¬Jﬂ|‰æö3Fã’vFgà°∞ÀòÆ®√ñ[Ôwqwh¶ﬂÊDAÄÅü#CÈÕ!ÊÑË{_wWà97›3b√œ˝°Ø\6√:k;ê∑òÈR6`9m-Ÿº‰ùs¢ÓÌÈl‹ﬁz6Œz⁄Ê9‰pH9ÌÛè+Û»ë1»sØ‹L⁄)Åçú¡Ö∏
	‰‹õéô´ÕDƒâ"!ÏÕå∑Ç∞æ∑Õbàb{µÎò;hÁ\Ÿù]EPàΩ CÂƒ∞ù•~ÜÒ˜Æµ<‘^XÆwW3"9ù~] #ËÌÕ˜}6#.∆Œ4∏}ÄŸ¸∞Tv±vﬁUß∆ÕrﬁT‹Fvj€ÍÁ.
À“¨ÿÑ<˜*òiÿ”á∂;G∆¨â«˜Í¨@{†¿HΩ!-õ!CüÜ3Uµ5ÆŒ5Ù}Â`dœ…ˆÁ"ñÖ›óæ©ßqB‹R7;∏ãπNr;36›îûá5≥g‰0!¬ÊYÑxŸJÊÓ«ÔûÚƒ‘‹ÓC á˜ÈC«bjàÛ±7r\À≠Œ˙/€,ƒŒ$»hŸ÷~»ˆAu˜hùg|cﬂBiHËÂ∑⁄ô)AL∞€∂7hdã™⁄1‰åvÛæÍuévm≥øŒ 
€AøÈõ L™:¸ÆÍÚƒﬁ˙≠ı‹˘a
VïÃ·`Cí˜5ª-á πÏrÏ&´{x*‚`x©∞˚]l±∞)Ìq_˚!«ì⁄t‘B:,{üvm¬BRN#Ewﬂ\Ÿ§7në{ﬂWfÏ	ùÀ5Óûé{Eåa›#&'*¸c∑ıÓÏÇy´ 3+ vûPﬁ}ëÇjÓ	ëTqes˜îD{~ã§
ˆ¢Ÿ<"&Yö)á µ∏?CÅ9æG@Ö;«¬l†] ·rÊ6œÙ∆”ÛÿtÍ(lîCÅôæA@éıîóë:€ıÜ]TÉo	VˇàπâmmÔ/˛1{ÿˆh:·wˇ0.∂Ô#€£ùr&wœ’_û[áˇä≈Z!Â©1I∞èÕ
˛?Óz‡¬ÊSjuÊø(«rQ‚É˛ô‘´±î]œù’ªΩ9"°⁄Î˛\O ˜≠~œ§Ò<é Æ?Û¡î√ˇ∏∞˘* ±ªm€§FúÜ·≠ÁJy9<äaπoﬁörÿQﬁ„LÏ¶Ás>n÷	yg`Ω≠Ë]•ÏÖôóEúô˜á¬«q5®úé≠’á.aO–+Ò√¶1,{ÎÍÆÓªêÌMd∂÷mÓÖ“Êk*ï”Ã¢
£(LâLlÔPˆ±ˆºâíÚûU°<ï•ë∑¬,¥x ±•H•Ó]>∞ù≤‘√Ù]w^v96ÅcÙåØ†Ç©∆-∆ƒND»—Ê(Ü,˜-·B9‚Ñr&bVÒ û¢ú…µ∫≠îsp¬MÚàâCª´]l)&aY∂bz¬≈òÕ3Úìæ
¶yfÈ¥ùÄïÁ	!ˆ€Q∂ü!hâA<T`Ó  ò¡
‡FF[¡⁄7&≤¶b!kå
äQwB÷ò(e"sp8%kqd◊v∞ÊF¨õGR¡ö„„—⁄AèXK7á8Ó`çnÜë˝`JJ÷Ö:£p¶Œgß…Á∫´X}‹"ë÷ê∏∏≈ƒ∏
ø8,p√ì7N$)pKXcci:*pCï∞Ü·î∑ïaÔií2·mï˚ﬂûÜ*o√übÁ'§ºÛ6[zÒ6œ†ê©Ó)øxõGÖ	∆ŸGf|Ò6R>,ì,‹Ê…|0≥€î/‹∆ıÏî
l„\™tGˆ^`Á$ å£=∂ÖÑÍ∞Z“!∞-†K˝$y€0òiÅmÃp¡Ü⁄∂aÑl´¨!∞-—Ä£~Åm∞qt|Ua[∆v≥∫Óß|¡6ÏË„<Œe`ÛËj€`ÌqÙ…‡l√ÆÃañL@"∞çª>LP?Âm„·¶≤&›⁄9∂æajm—∂ÅπtLz∂hõ7Q⁄÷h†1O¢¢¥ç(≤∑”6f¬2 m√áïµ…um∞K€ôZ^¥
ü'π⁄f™⁄fö#¥
nçl{ÙJaÔÑh|¬π€ê`
l∂¡∂;Ç≤6/ÿfÍ^¥
&∏ˇ=‹∆cƒBìá-‹C˜9 B€"æc2f°m·(w¨ìŒ	mÀÃÚÊIo/‹ñáÎ
'õ[ºç)88Ë·˚î∑qƒ∞V‰ù∑a‰]heö«‚m–tÈÑ]CÃ¥ûÉÀ=ËÌúí¶|q8[^8\ ‰pSÔN0bQcq¨Xˆ√lŒ≈Á0ÖòÿE|πÚ9∏ÕûIµÜ¸‚sÒ7fÍküc˝ ÕMÄv:∏I∏≥îÁs:ÃbƒE0Î	÷.@GGãπ„ÁNX]!÷Ãi÷#Äı3 òÌ@ßrt‹&Ô&Bòt,aËAù´yOS~:7ñÌ6sBË0€Zs}nÖ°´<ÄÈáÁBg_Ñé;;¯”6≈BËL”OBg˙)ÑŒÙGù©D	]‡ë7Ê†!tTú˜î/Bg⁄.ÑŒ∂g:nCó˘\!tÊπã–Ÿv.BgÎBó»•g®aù∂_TÖ%¨Mp%åŒîø [D/ißtåõ£cNÊΩ¡t¶ôäÈ‡9@µ«ŸÊéS;∑ÀÔ8ŒT/8Nµ©8n0/Ïá|·8ƒ≥òö„tåÚ83X¬„Lkî«isî«©íï«π8’¶8€≠≈„L5¬„å|9[Ω 9rt∑àÇÔDÓ"o⁄%oj<Jﬁ
FDT·îﬂ…õï/Ú∆Ω$‚—ì‡	yS#TÚ∆iÊÊ1Cÿ¥_Bÿl;Ö∞È\Q¬fûªõ1%l⁄/!lFˇaª∆k#lW˝J“¥=B“LÒE“LwI3LHöô+Ç“‘∆•ô∆,î∆<ÎPö©g°4€úÖ“Ã†(J3œî¶ Wf¶⁄ffû´ÃLçPôô∂GòôY˚éŸÁ^pLßê¿1[z¡1«
±gÈß¸N«¨\ò©_òiΩ¡cÚ\¡cÍèô˙è°i®¶LÌ3œ<¶¶ØxLÀ+3ÂèÈ®3£´|L€Ø|Ã‘#|L≠M˘òŒ-·cf™+3ı3˝Z|ÃËÛŒ«¨rÑèÈ`	3É+|Ã6R¯òQÇ1ıß
»L˝êŸ˙ ≥Â 3É"ÄLu¨ÑLWo!d™2%d∫∞€ˆß¸"dÍêîê©ñïêÈP)!”°UB∂ïøô©12[ojB◊Æag¶~ag¶_¬ŒLyag¶˛≈ŒÃ®+;3Ì\ÏL˝æ∞3≥H+<3£ª‡ô}¨¿3ÒÀíIÛí©±)$Sı($”œ@2ièÅd¶˛…ˆÚwH¶Í7êlì_êÃ‘#êÃËaA2’øÅd¶ùíÈ0*$≥zHf $€‰wH¶”Q!ômœÇd∂¸Ça∂_ÜÈ∫k†ó©_†◊&øC/µOÖ^¶ºB/mèB/G°[2€
›⁄ä_tÀ»›2f9Ü≤ˇ(øS/3åwÍ•^©óÆñÜzôæ^‘À®~Äõÿ«z ûViò1eK√.Kf.!ÖπÕ3Òà•8Ï≠∑ÙlïøËô¯CœdqZÙló^òÃ‘-òÃÎ¬d∆)&3ı&3ıXL∂Zø0ôÈ;&ªÜ[1ô÷Øúlì_úLg°Ç253eª¸e™e¶∏Ä25@b¶ôñˇøÄ2«ÌÃ…∆û¥å·uΩ¡~Ù7?√Ãx ≥&[f÷ÈC#¢Ãå©‚^˙~ç7  »:
2Ûn8ån£!bNÖfûëtç#wnÆ£1B,ìP(5cB
;Á…¡.j#ﬂ¢'_j∆|N∆0Ì‘,¡~¿èÛ"BÕ°Fx4FØ©0¡ÁéjÙööñjñ1wù‚a©ÙT—≥1g
5#&Í'ƒl∆˜íãc√f∞√ø9qö`3Ê…[µ‘å˘gh/l∑‘|g¯&º—[j\±R€òY‡:ôbåMÔ®—€aﬂ‰Ê›µÕËYC:ôã‚1ÏÒ¯ô¥øXƒº-#∑x,¬Rõ´3e/|,
du“4πãF{ŒÕ;jÇ«–.Ë{≈c}∞£…Íèﬁ˙…Ûí–1Ï›Û†›«F«ò(™¶#N°ôwÀ.:VáCú3ÖéE:–q—ÊÿÆ¢a»¯ö«YÕ¢càXK¬LÿÈòïÀ]4^_ ^?∂ªhô®¢O÷∏ËX§≥√∂f6_È¥¿ºÃ√]4ÿm:/+
3’»U¥à)à
Ò«`∞ÿvﬁP[påô\8°º√1S^‡XÏº9/“	#ˇ∆ÃÒ≥∏‹D+º°VÊ˝ØÎ&oÈ•2Ø≈	c‚12l9∂ªhp•X·˚N«`≠êˆykPËµTÎâêı2⁄x}gò≥AsMp¶∑
ÉV[L~^[∑—9˚:Ô *´Ã4µ∏„1T0'[÷ÎhXƒ2t?Ôù]xÃ4FÒX'ˇn*3r¡cµ‡¸∆BjòiŒ¬cZèπæÜ·q‚ƒQÇ«0√
—◊ê/<fÂÇ«`•ë\o◊ª:"’˜èqÉHÚè—”29Í'ªØÎ¡,Á€ú∑˚kòFµŒ[`≥ÌT<Ü)ELåßxå>C:Ôû-<∆Ã∂Ωa	3Úèa‚°µ'[xÃà
Û˘ÃcËù4∏—´òw√‰Nö>Sâ[ã®tﬁa[ƒZÇÂNºÆªg~Pú:…ì‹=3ÚE∂l=B∂∞\c›û	Q%[#Í√~˜Ã®A»ñB%[Œ÷œ√Ÿ˘"[™{ˇlç∏^@+ÉîIûÑlmÚÎöy¨/Û\!^ÊπBºËÃ±¡ ß¸$^FÀBºå\âój”\@[≠Q‚àçO~ ^Otºi∂àóïõhÁx5!^|7Gm'bZƒã€∑0ºTôºLÌºLÎlôjÃM≥•Ωj&3Nyóπ.£cÂ]XÀπÔäß¸‚]⁄|Â]:£ÌM≥’|·]¶ôr—Lµ†ÃTO≥s3mö#xÃtw·1˙.ÏxL∆PÔüÌ,:f,VÔü©Q
&’Î53UéΩf∂Z/pLá\ØôÈ4îkfjØzÕLùö¿1#8¶mókf:"ñçI#Âöôî∞1Æ
-µ÷O˘≈∆L˝¬∆T≈zœL-«ﬁ3ªöoëŸAEf:$äÃ¥[äÃT˜zÕLáPQö6Á"i:RB“ånÙöô©\ÓôIS]⁄ãfR^HöŒ*!i∂=B“L{Ñ§e
IS[íf¶õí4-Ø$MMVIöˆWoöiøî§i˚-I[˙Qí¶„eoöI˝r”LçGIö8A{—LäH3›ΩÉ4”Wi¶-“ƒ Ì=3).MáP9ö6]0ö©∆ﬁ3[å¶≠ä¶=ä¶s_)öéìπgvU.ÕX±B4Sã@¥M~A4’ºB¥M~A4’çB4’ç¬2#X¶Ê°∞l+¡2UÉae◊**3µ*3Z∏PŸ.æÆô%*”©y¡›á].˜œ4HSÑ&.¡ 4Q≤Ah“-É–§˝Êûô¥ﬂ†2Sè 1”Ab“/Éƒ6π ±kÕΩ1S^êÿV^êò¥SÓçôv
3z$∂å«±e<àii·a¶rπf#ó√L˘u9L›Ç·dF9¬…6˘u9ÃÆÂdW˝¬…L{Ñì©'QN¶’+'”±RN¶jPNfö≥8ô}¨‹Ì_òÃ¥E.áô.≠K`ZÖ–0+æ`òN√ViaaÊëãÖ©¥^‹,/,LGOoí…33Ω.íô¬rìÃT-àÃ4Qô!Ad[˘;"≥]Df "”∆õãd¶¯ùêô…≠ÑLõ©ÑL
O	ôá2ié2’¶2Yñ- ìV
 ì(œÄ0” À S8∆ƒ’ÅêÓ¢dm‹$CÙüËƒHπ“√£µÅÕ¸œP2¬(Ó€∑õehIr—m7Àb–‹–öP2Ñá°c£6ƒì1πI›ˆb[y\ad|÷ÌyK/ñ1„ô‹|Ÿ¢^,„%WåÂv±,º‘˘RB}c#5À˛«v±ì'M€Bπ∆ú◊¡, É«)#©©ÄENÜ	∂ê!T@≥∆]Y·“ñ'ì@Vô)«ûi Â=éqTü˜íÃ˚°2æ3w¥GﬂÃH∞√KñnÖÒ∫Í4_tßoTÏÿ	ó<Ÿãê æñæ§O&≥áñ∑ﬂX‚›õ‡|´€
$éN≈ÄO •–;a®9Ô/‰ã|Ÿ"ÃxæêoaçÑ›F·ñH‰pké€êc#	é^<üwX‰äM™ùl@í˜Ã/˚2ﬂ IwÓ°∏ô˚ñ´$Å√;_÷'9Óë”g*{^›∏í–qæùÒ~cﬁ£‡∞!tI◊«Œ{ëÔNÏ„5Ôm∂ñ¿•ú˜c4m ú
‡ÿ“óË+<€,Ø	C8ÏzﬁY7/âb:-˚¸êã¥Y?;´…¶ÃÏ˘"9„<é¢Ã˜Øöåò˚ÃYIÄé?êúvóà`]sG∏ˆft©Öômﬂ"ÉÔÔ°Î=DÖf!Òf‹√^#wÂ7øŒ<{OÛXà∏oà˘™“áã√*ˇ3∏ı|^.ùØ‹uw'œWÓü™˚π√L¢é∂Ìn≥%œªæ‚÷πÁº{ßn›Û~j
€Öaÿ=|Êú&‚◊ˆ6gõ¯uÓ≥6õ_«^5ùÊ-^ùªôyN‚rÍéª„:›®Sg»G5˝±8uÚ#Ê’WΩ-åÌÜ¥o^=•ò|[ÊÊ’#mlÛÍ|ùgH„Ëáπ+ÃªÑ'06ß∆‚0-ÿúz@áÂ'ÏóÖ˝xr}wˆï˜RT‰≤0º,&Vﬂé7Uæ|”Á|ï™d‡î``∞/<_T£{∏πÀ;å1›]∫‡wxq˛¯ÅW∏&àßãﬁÌ¯∂j˜pãì'"òÇ-õGÁ…ïÁûL=:ø"’Iﬂ≈°g¶˚f_≈ù”¡5Ìo eû5¥∞{s8#Ã≥∏_ËkòoÚ]§ë@7Ò1”ô_êp‹;Ñ«å€'	Dyliû˛]TéÔ#e˛|¶.5#àÌΩ∆8˘íº?ëÀß;¡‚HDµ¸RäÈŒÂS„ñ•ÂÈ∂
Y¡åji¬ AëG ÃJŸ+4pCß˚◊¸;öøj2’\!RÿØA–`†mOZ¬Õc\Úy-¿∏yNŸ3ì≤“F<$C?ÿ3æºéï„⁄Û^{€ÃúgIeÔA/üÚ˛∂:sz\ˇÇ¸œ·‰”˝ÌÙpÚ1ŒSm·ﬂô1ù¸œáÓX‰15|<_f}|?ﬂ´´.cÄßé≥DÍ‚˝ék€;!òc≠¸Zî-tÁlÂú⁄\<Ã∞Áˆw≠;ÜÉ|èπuÚÖAÎLŒöWB0YÚ£ìáqbFœ‡z9˘¿xáf≤yyûù„;⁄ÊÂ˘fezˇ∂yyæS C0ô9‹∆◊√!áÕÕ√Ÿ0jjmsÛïÄ—=º¢ÒùDnûŸª‹yÁ;¯¬oÎŒy.Õı˚ô,=ó÷§ôgh‰¸÷(¨ÛXÜæ6ú/—'Ø;ﬁ€~Gı9_∏∞MEÊR"~æ
`Ç‚íÈ¯‚
ÎÂc`R"¶˝ÖŸâ›ªøô]é!†èÛHì# |◊ÈπG—”?
}ûÆù€¡∂¡a•x∏è£Âπ€È‡‰†ñ€^–I8`„ÛéçLßH„yBÉyT	CôÃÌ
Ê3Õvæ8›Û<Fõkà{0`¸É]ø7oÊM¸V†ÛéQå˚aÅëı+˜ÎÆãŒÛ]ˆ0ÆÖ2¬ÄØòºZ¯3µÛÁÀ0ÖÏésõÆ|ÄÇb¸˙I‹dR∆còk¬"bÃ¶`gôw∫Ë£Ê	.E‘_¬≤?/ê¨l6‰‰±á√&6·û18ﬁﬂC˜ÑQ‡ì–Ä=E <“¥ßhTnøÑgïÁÄã?æOd~e≥3_îu~c˝˜ˆÎÒãáØ¥ü≤≥»cy«gü_B‚ÕWê|sˇÜê0æ!Ñ')«7esÇÁ˘m2ø{˜’˚Øè˚Í_æ˝Í_ø˝Òá˚óÇ|ˆõ8W©oPÕwr¯∫°{ê>=!Æ§oÂ)‘Ò≈.ÿ+›ÊógâòKO∞vƒ(*Á—–{a¨'’s¥UòÔ%ﬂ=-ÒH@ÑQÈç¥¯Ôê'ÒljfÖÂ*6ÔÿÍÛÁ˜OÛ`è<û¢nÍÎ◊Òg¶MÔÁÁ´·´"È¢’œªß‚Ω¸‚ÔS9^˙>ï˝˚j0±#ÅuÜq†›ÎÁÕB˛t}1ç˘Óœ¨0¨ªáÛÀ>˘o_ˇ˚∑Ô~¸’ø~˚k~ı√7øˆwÀmÌ∂Ø¨:^~eU?oHÊ”\º7Çèh&}◊¸#iÁªﬂˇÔ/6÷\¯àk„~¥ø
˙u∂˙˛Òó∑ô)~ÉôiÒèˇÁ«Øﬁ}ı√Z˝r∫«K9›G˚‡n—9QΩŒn|≥˘éŸ˘ˆΩ—û•?-z|É.ƒ3i∏«s—˛·+Ô~=æ´ë;B;˘“=ˇ“=©`¸‚v~Cûgfp~
“¸EzÓ/⁄sø¯’¯O≠èÄj=¸ô6πènS|Ó/Ísø˜ØÓ˚âSÜÍu◊wBπ√Ôæ˙˚?˛Ó´˛ÈˇﬂÔø˝Èè_˙«æuÒÛø>˛Ê«ß/˛°îoàÇÏP<S”æ˝Ê˚Øf=_<oo+Ÿtºîl˙ÄΩù'ññΩ-¡GŸ[)A{Àœ˝≈≥Ü¯¥∑g€T˛Ÿ€µÔ=~Ÿæ˜È47~Kú1∑%¯(scFÓ?ûπ˝≠ÍŸ6Ö7≤*l∆øV-¯è6´/û˛/∂G
endstream
endobj
11 0 obj
9203
endobj
16 0 obj
<< /Filter /FlateDecode /Length 399 >>
stream
xú=í…ë›0DÔä	L±qâÁª|ö…ˇÍ◊îÌÉäI4z·Ã∂aˆcYüi=á˝ÚÁñµÏÁÈë6∑}?µõke’√æNX
Vœmü'ÎPÓ≤ÿ˛B9˝∑¯<>ÎÔ^ﬁ¢Ã˘°naú∂nÏK≈ó0yúπHmán˜6w
ãt• cæ.ódÓ~ãœì2á@}Y&ù{ä‚åÛ<¬r+}"[Äo©Õì¯a	˘Tß€ù‡/ãÿò1Æ¿ÕÍµmjk6ßÏköWhâ°π*zÍFÚâÏbiI:
Æ‘ñY—∏ËÔ†9ãÜ∆$ØN(≥D®V¥ÕwßÜsD¸È‘ò“h|®>DÎpkJVè7ÓÔˇ¡ì7¬?o•ª$_»bëàcÉÜ≈ãﬁGñﬂöC“F ¡≠"JÂ"_∆U€◊*u‚‚ƒsÛ%”±ÙÍzÉû…IPπﬁ’5Gï£ÿ·„ºfΩ˜Õmc¶btÃªàÿæ∆O¢r	‘÷å"(ΩŒÀçHˇÈˇ<øˇ ôæï™
endstream
endobj
17 0 obj
<< /Filter /FlateDecode /Length 87 >>
stream
xú5ç¡
¿0ˇô¬#ƒ ŸßÍ´›ˇ[H‘è}≤å±XËPKq
¬;.6N›¯6âCOfe$çe∞QT'áƒ'dZí±≥≈æùØ≈v¢«˛'Oª?∏Nƒ
endstream
endobj
18 0 obj
<< /Filter /FlateDecode /Length 52 >>
stream
xú32∑P0P06FÊ∆
Êf
)Ü\Üf.L0áÀ–§(áÀB¡î‰p• ∂*

endstream
endobj
19 0 obj
<< /Filter /FlateDecode /Length 299 >>
stream
xú5ëKn1D˜s
.…¸å}ûâ≤À˝∑y–ôEãjÃß™ÿj≤$∂|©KÓÕ∑‰[_ñ1©ﬂóﬁ5H˝ ]&ëÚ~Ìê›®~:ÿ*≤
¢$MÏîÏ∑C∫J|_π4¨’îp#Ø‘F1„∞|1#⁄Â≈6(Æ8Ÿ¶‰˘DVÿEå5}πzZ≤=ˆ##–’—≥{-ƒÂïgr±k^>–K-—@€%jåîVt˙ÁRG⁄!ıÂL{¸˘¯Ñ¸1]ÌHa®î*äî1∑Eµïl6Ÿ8ÑÖªyª
r9xŸ^á6É]G){F1{üóF]K[–d#Œø;Q6|É9ŸélAU#;>û[‚˝8jﬁ›1'Ï~=5”!\ ·pﬂ‹πSÚør.'¥åj|˚®ø~˛ ¯nT
endstream
endobj
20 0 obj
<< /BBox [ -1016 -351 1660 1068 ] /Filter /FlateDecode /Length 218
/Subtype /Form /Type /XObject >>
stream
xú5P;é!Î9Ö/∞˘Ái´}˜o◊	o
úÿfò/¯J|Üûã4™
ÁyÜÏÑmá§¡, !–eıb‰Õqe7õ!≤{∆∞'îóThÆ*œ0ÒFç-∞#§ˆ]≥xÃ^Ë\t%|9EieMö–f\[n“FÌk¸çBïoüëq˝çÙö-./J*ŒD,ZÚ@ê}UãSb2Æ˘Ç¨;4J∂¸∞ØÏWe`ŒiùÊµﬂÛvÓ∫ı›_°˙Ø∆X”·¸·gË§a~ÜÆh„oîg¸˛¶?O≥
endstream
endobj
21 0 obj
<< /BBox [ -1016 -351 1660 1068 ] /Filter /FlateDecode /Length 303
/Subtype /Form /Type /XObject >>
stream
xú=RKÆƒ0€Áæ@% |ícº3Tö’Ã‚›ÛL€7™TS&øPü˚}~∆°Ü√§:·Ö˜0˚è4:€QB˜ÜFïË–5q23°E∂1ÛF÷=[d
*}^±:a"(ÉY!ñ≥·SµÉÈUò≈n‰]MÉ±&‹Öµ-bœ§±øë“üeG¬ﬁ&:PıÂ™c$y3≠A‹ÎIpƒ`«≈Bù®lZ•„§¡Y§g‹ﬂ˚è>D:3bwuî¥V”â’c9◊A≠ÖÉá4p‘cÂ‡|m"Mrç¥œï_ÃdErâ.p:¢9ßIˆo»>=∑puòIÔgãkµ’måﬁZ x{∑∏—RG∫≥≈µ¸◊‡ıñ[©ó/‡û£g∫ˇáÔèÛØÒ3˛ ”ïou
endstream
endobj
14 0 obj
<< /BaseFont /DejaVuSans-Oblique /CharProcs 15 0 R
/Encoding << /Differences [ 103 /g 107 /k /l 111 /o ] /Type /Encoding >>
/FirstChar 0 /FontBBox [ -1016 -351 1660 1068 ] /FontDescriptor 13 0 R
/FontMatrix [ 0.001 0 0 0.001 0 0 ] /LastChar 255 /Name /DejaVuSans-Oblique
/Subtype /Type3 /Type /Font /Widths 12 0 R >>
endobj
13 0 obj
<< /Ascent 929 /CapHeight 0 /Descent -236 /Flags 96
/FontBBox [ -1016 -351 1660 1068 ] /FontName /DejaVuSans-Oblique
/ItalicAngle 0 /MaxWidth 1350 /StemV 0 /Type /FontDescriptor /XHeight 0 >>
endobj
12 0 obj
[ 600 600 600 600 600 600 600 600 600 600 600 600 600 600 600 600 600 600
600 600 600 600 600 600 600 600 600 600 600 600 600 600 318 401 460 838 636
950 780 275 390 390 500 838 318 361 318 337 636 636 636 636 636 636 636 636
636 636 337 337 838 838 838 531 1000 684 686 698 770 632 575 775 752 295
295 656 557 863 748 787 603 787 695 635 611 732 684 989 685 611 685 390 337
390 838 500 500 613 635 550 635 615 352 635 634 278 278 579 278 974 634 612
635 635 411 521 392 634 592 818 592 592 525 636 337 636 838 600 636 600 318
352 518 1000 500 500 500 1350 635 400 1070 600 685 600 600 318 318 518 518
590 500 1000 500 1000 521 400 1028 600 525 611 318 401 636 636 636 636 337
500 500 1000 471 617 838 361 1000 500 500 838 401 401 500 636 636 318 500
401 471 617 969 969 969 531 684 684 684 684 684 684 974 698 632 632 632 632
295 295 295 295 775 748 787 787 787 787 787 838 787 732 732 732 732 611 608
630 613 613 613 613 613 613 995 550 615 615 615 615 278 278 278 278 612 634
612 612 612 612 612 838 612 634 634 634 634 592 635 592 ]
endobj
15 0 obj
<< /g 16 0 R /k 17 0 R /l 18 0 R /o 19 0 R >>
endobj
26 0 obj
<< /Filter /FlateDecode /Length 87 >>
stream
xú=éª¿0C{¶`Û	Ü}r©ú˝€Ä?i–C:N∏	6œ—Ì¬ŒÅ7AÓE/∞.oÄ
!ã$˘ˆŒ≈¢Vô≈Ø¶EÍÑ4Iú7QËNãJÁ„Ùx>∫uz
endstream
endobj
27 0 obj
<< /Filter /FlateDecode /Length 338 >>
stream
xú5RKí[A€øSËÆj˛Õyúö’‰˛€Ï¨†Åê8»ƒKQçr≈yÇÒ:ÅøÎÂi¸>ﬁÖ‘Çß"˝¿µiÔ«ö5Q∞4b)Ã>ˆ˝(!«S„ﬂËπHfd2r à˚µ>÷õL9¸§is˙(Iz-ÿ›v|YêA“ìñÏ‰áu-∞∫Mòk"9µ25œ«û·2û#A’, Iü∏OåH3;g-yê·x™/~Ωç◊2è©óU2∂	Ê`;ô	ß("ø†$πâªhÍ(éf∆ö€ÖÜí"˜›=úúÙ∫øúD^	·,÷éz 2';
J†jÂòaΩˆÖqö6J∏S”Ì]±Øﬂg&a‹Ê∞≥R2
Œqp/õÃ${›1aáò˜Óåƒº˘]l\πÃπ&”è˝(⁄H◊Á\Mô≠(·™‰â◊¯ˇ¸ﬁœœ?ê7}±
endstream
endobj
28 0 obj
<< /Filter /FlateDecode /Length 304 >>
stream
xú=í;í√0C{ùÇ»å¯ì‰Ûd'ï˜˛Ì>2…VÄIâ (/uô≤¶< i&	ˇ—··b;ÂwÿûÕÃ¿µD/À)œ°+ƒ‹E˘≤ôç∫≤:≈™√0ù[Ù®úãÜMìöÁ*K∑û√µâÁñ}ƒ74®uçK¬
›’hY
Õpuˇ;ΩGŸw5<õTÍ‘èQÊ˘!O¢áÈJ‚|<(!\{0F‰S—@é≥\≠Ú^Bˆ∑≤¬AjIÁ≥'<ÿuzO.nÕdπT¯NQÏÌ–3æÏJ	=∂·XÓ};ö±Èõ8Ï~ÔF÷ åÆh!~»W'Î%`‹S&EdN∂Xnã’ûÓ°(¶sÜs ÍŸäÜRÊbW´;o,/Ÿ,»îÃ2FßMû8x»~çöÙyïÁx˝lÛs;
endstream
endobj
29 0 obj
<< /Filter /FlateDecode /Length 230 >>
stream
xú5QIn√0ºÎÛÅ ‚.ø«AOÌˇØ“	``hKúÕxâ¡œA‰∆[÷åö¯õ…]Òª<	∑Ç'Q^Ü{Ÿ	.oó˝8Ã|^Z9ìO2 ŸÙD»`ó@Ë¿Ï‘aõi'˙ÜÑœéH5YN_K–K´(OŸ~ßJ¥≠ÍœÌ≥.¥ÌkO8ŸÌ©'ïO û[≤óçWLcÙDÂ.≈ÙA™≥ÖûÑÚ¢|≤˘®!]¢úÅ'£@;∞Á∂üâWÖ†uuü∂ç°)Oˇ645I"‰%úŸ“∏[¯˛û{˝¸¶TSü
endstream
endobj
30 0 obj
<< /Filter /FlateDecode /Length 66 >>
stream
xú36¥P0P07W–544U022P042QH1‰2443sπ`Ç9`ñâêa$¡r∏`Zs¿: ≤P≠9\i M8ı
endstream
endobj
31 0 obj
<< /Filter /FlateDecode /Length 227 >>
stream
xú5O;≤!Î9Ö.êåm`œ≥ôT/˜oüd≤
˛HÚÙDG&^Ê»¨ŸÒ∂à¯SÒØ=Ì√ÑÍ=∏áÂ‚Bòa$ú5Î∏õß„≈ø]Â3÷¡ª
æbñ∂0ìıï≈ôÀv¡X'qN≤c◊Dlc]ÎÈ÷L(!ùÌ0%»)}≤£å9:N‰âÁb™≈.øÔa}¡¶1¢¬WO–dPñ=Ô&†Ùﬂ’çﬂI4ã^2ë`aù$ÊŒYN¯’kG«Qã"1'§‰2“úÆb
°	≈:;
*óÍs ›>ˇh][M
endstream
endobj
32 0 obj
<< /Filter /FlateDecode /Length 245 >>
stream
xúEPªçC1Î=`˝,{ûwHï€ø=JFpÖ!Z?íZòà¿K±îo‚GFA=øÖ‚3ƒœÖAŒÑ§@úıôxÜ⁄FnËvpŒº√3å9≈Zp¶”ôˆ\ÿ‰ú'ŒmîÒåB∫ITqTüqLÒ™≤œç◊Å•µl≥”ëÏ!çÑKI%&ó~S*ˇ¥)[*Ë⁄E∞H‰ÅìM4·,?CíbÃ†îQ˜0µéÙq≤ëGu–…Ÿú9-ôŸÓßÌL|X&ôQÂ)ùÁ2>'©Û\N}Ó≥—‰¢•U˚ú˝ﬁëñÚ"µ€°’ÈW%Qôç’ßê∏<ˇåüÒ˛é†Y>
endstream
endobj
33 0 obj
<< /Filter /FlateDecode /Length 392 >>
stream
xú=RKn1€œ)∏@•Mrû©ﬁÓ›[õÃT™
/∂1îó©%?Ííà3L~ır]‚QÚΩljgÊ!Ó.6¶¯Xr_∫Üÿr—öb±O…/»¥TX°V›£CÒÖ( -‡Å·æˇÒ®¡◊∞Ör√{d`J‘n@∆C—HYAa˚ëË§PØl·Ô( W‘¨Ö°tbà
ñ )æ´
âò®Ÿ†áÑïí™“Òå§[¡]âaP[[€xf–Ÿﬁëç3Ì—qYk?=È£Q2µQMg|Ò›2RÛ—Ë§“»› CgœB'`$ÊIòÁp#·û€A1ÙqØñOl˜ò)Vë; Ω˝ﬁíçœ{‡,å\€ÏL'—iß≠æb˝É?lKõ\«+áE®º(~◊Aq|X≈˜d£Dw¥÷#’h%¬ŒÌ0Úx∆yŸﬁ¥ÊÙDh£D‘é=(≤≈Âú∞ß¸¨Õ±û&{o¥èîÃÃ®Ñ‘vz®∂œc‘wû˚˙¸. °
endstream
endobj
34 0 obj
<< /Filter /FlateDecode /Length 71 >>
stream
xú≥0∂P0P040S047R076R015QH1‰	Åòπ\0¡0À®,,ã`AdA,#SS®¢√Æ¡Ç»¶ ÎÁ2
endstream
endobj
35 0 obj
<< /Filter /FlateDecode /Length 247 >>
stream
xúMQªmD1Îﬂ\‡ ÎkyûR]ˆoC…ê¬ °/)ß%ˆ∆K·[æ‰ëUC?1Ï3,=…‰‘?Êπ…Tæ™õòPb·˝hºt/"+ ﬂèesŒ˜‡£ó`&4`¨oI&’º3d¬â°é√AõTwM,ÆÕ3»ÌV7≤:≥ lx%‚∆ DŸêÕ`£å±ïê≈r®
íZ`◊ÈQãÇ+î÷	t¢÷ƒ∫Ã‡´Áˆv7C/Ú‡®∫x}ÎK∞¬Ë•{,|ÆBÃÙL;wI#Ω¶fRôùëï:=b}∑@ˇüe+¯˚…œÛ˝(\*
endstream
endobj
36 0 obj
<< /Filter /FlateDecode /Length 90 >>
stream
xúMçA¿ Ôº"OPD–ˇtz“ˇ_´‘Ω¿NâEÇÙ5jK0Ó∏2kP)òîó¿U0\⁄Ó¢ ˛2ILùÜ”{∑É≤ÒqÉ“I˚ˆqz ´˝z›“"X
endstream
endobj
37 0 obj
<< /Filter /FlateDecode /Length 338 >>
stream
xúERKr≈0€Á\ 3Êg„ÛºNWÈ˝∑ïp:›<Ù	2=eH¶‹6ñdÑ‰Ú•Wdà’êüFéDƒﬂ)°¿ÆÚπºñƒ\»nâJÒ°?ó•72ÕÆ–™∑Gß6ãF5+#Á CÑzVËÃÓQ€d√Îv!È:Sáp,ˇC≤îu )îmAﬂÿ#Ëo<‹≥Êr≥πLnıøÓ[û◊:[±m@	ñsﬁ` ƒ√	⁄ ƒ‹⁄ﬁ)(U∫äI¬≠Ú\';P∂–™tº7Ä9`√í≠◊ho √>Ù¢F≈ˆ†®, ˛ŒŸf¡ﬁ1…H∞'ÊN=q:≈ëpI8∆@ä≠‚∫Òÿ‚/Æàö	u:eMº¬û⁄‚«BìÔRq"n]EµlOÁ	¥?*í3b§ƒ—	ë‘íŒóı–˚∏âØçƒÊûæ›?¬9üÎ˚∏É‡
endstream
endobj
38 0 obj
<< /Filter /FlateDecode /Length 68 >>
stream
xú32∑P0P∞4Ü&
Êf
)Ü\@æ©âπB.Hƒ ≥Ä¥%úÇà[B4AîÇX•f&fI8"ó …¥Â
endstream
endobj
39 0 obj
<< /Filter /FlateDecode /Length 81 >>
stream
xú=ÃªÄ0–>SºB|ÄÏ„±“˝[¡D∏|’!‘
ná¥¨Kwì}Ízµâ§»Ä“Sj\Nå®i}©}j‡ªÊK’â?ÕœÁá«k
endstream
endobj
40 0 obj
<< /Filter /FlateDecode /Length 45 >>
stream
xú32∑P0P∞4Ü&
Êf
)Ü\ñV.L,Ã—ñp
"û ü}µ
endstream
endobj
41 0 obj
<< /Filter /FlateDecode /Length 255 >>
stream
xúEëKí D˜ûÇ#Ä¸‰<ôöUrˇÌ4òL6vó®˝ÑJ#¶,Áy0˝»ÚÕd∂Èµ´ùçä"Ã‰*ÙXÅ’ù)‚ÃµDµı±2r‹ÈÉ‚
ÁÆúT≤∏Q∆:™:8¶Á ˙™Ó¸∏, æ#á2l÷96pÂ∂aå£ÕVwá˚Dêßì©£‚vêl¯Éì∆æ ’∏N6˚Í%Ç~°	LÚM†uÜ@„Ê)zr	ˆÒqªÛ@∞∑º	§l‰»åAªNÆqÎ¸ﬁˇ:√ùÁ⁄WéwÒ;Lkª„/1…äπÄEÓ‘Û=≠ÎÔ…ôcr”}CÁ\∞À›A¶œ¸Î˜Päfà
endstream
endobj
42 0 obj
<< /Filter /FlateDecode /Length 161 >>
stream
xúEêK√ C˜úBGG|ût∫JÔø≠!M≥Äß±@w'©µ—/mK∫>[	Œ∆xË6n5‰uÄV§„hîR}π≈iïtÒh6s+≠fzî£†:ﬁÌ¢‰r¶ÓŒ˘Gpı_ıG±ÓúÕƒ¿dÂÑfı)Ó|õQ]›d“cn÷kˆ™∞¥¨•ÂÑ€Œ]3†Ó©Ì˝©s:Ñ
endstream
endobj
43 0 obj
<< /Filter /FlateDecode /Length 214 >>
stream
xú=PªC1Î=‰Œ|Ì7œÀ•À˛m$ú§B6BîöL…îá: í¨)O>KbáºáÂnd6%*E/ì∞%˜–
Ò}âÊ˜›’ñ≥C4óh9~3*™”K6öp*∫†‹√3˙
mtVá±[ –§`◊∂ r«¡ôã"JMˇ≠r˜R‹Ô=o¢àîtÆ˘ÂÙÀœ-ºN=éD∫Ω˘äkq¶:
DpFjÚäta≈≤»C§’5=kµ Æﬁz˘7hGtÄÏâ„4•Cˇ÷∏«ÎáäRÙ
endstream
endobj
44 0 obj
<< /Filter /FlateDecode /Length 80 >>
stream
xúEåª
¿0D{¶`~&fü(ï≥ J‹pO∫{∏:2SﬁaÜáû,ÜSÒô£`5∏FRçùÏ£∞n_uÅÊzS´ı˜*Ovvq=ÕÀÙ
endstream
endobj
45 0 obj
<< /Filter /FlateDecode /Length 147 >>
stream
xú=Oπ
1Î=8¿z,[Û\êÍ≤ FR"@ÒëeG«
\bìé9/i?¯iÅX5GÙÑäaX‡níÉ,JWû-^ë⁄B]H¯÷ﬁ≠Ld¢<Ø;p'£>TYz@;DYÆI√X’V]jù∞≤Œ¬u=Ã™Â—'k)PTBΩtˇü{⁄˚ o/Î
endstream
endobj
46 0 obj
<< /Filter /FlateDecode /Length 149 >>
stream
xú5èK!C˜9Ö/0R~Ñp™Æ¶˜ﬂ6aZ		€/¡ÉëåKL`Ïòc·%TO≠>$#è∫I9©P7OhL3l“% tﬂ2û[ºúVÍÇNH‰È¨6¢åf^√—SŒ
õ˛À‹$jeFô2ÎT∑≤≤`Êµ<˜3Ó®\ËÑáù ∞ËN1¢‹fF~ˇ€Ù˛{20c
endstream
endobj
47 0 obj
<< /Filter /FlateDecode /Length 49 >>
stream
xú36¥P0P040íFÜ@ñëâBä!H ƒÃÂÇ	ÊÄY@¢8Æ&á+
 ∆Ë
&
endstream
endobj
48 0 obj
<< /Filter /FlateDecode /Length 157 >>
stream
xúEêπC1DsUA	∞Í±«—wˇ©˘J¥o -áØ%S™'"¶‹◊hÙ0yüM%V,ÿ&∂ìrAJ1òxN1´£∑°ôá‘Î∏®™∏ufï”iÀ ≈ÛhW3ì=¬5Í'MË¯ü<¥©Ë[†Øî}@µ8ùIP1}ØbÅ£úv"ú‡>Gô)#qbn
Ï˜ fæW∏∆„›7y
endstream
endobj
49 0 obj
<< /Filter /FlateDecode /Length 68 >>
stream
xú336S0P∞0¶¶Ü
ÊFñ
)Ü\@>àïÀÀ≥Ã,ÃÅ,#êñ.Cc0mbl§`fbdY 1 ∫“ r¯ë
endstream
endobj
50 0 obj
<< /Filter /FlateDecode /Length 317 >>
stream
xú5RKrC1€øSpÅŒòø}ût≤jÓø≠Ñ'+∞-@B./Y“K~‘%€•√‰W˜%±B>èÌöÃR≈˜≥œ-ØGœ∑-
Q=¯2'"‘œ‘Ë:xaó>ØN)xì Ø·_xîNÉ¿;2ﬁìë$¡öKãMHî=I¸+Âı§ï4t~&+s˘{r©j£… Xπÿ§+)$=âH≤rΩ7VàﬁêWí«g%&›&±M¥¿„‹ï¥ÑôòBÊXÄ’t≥∫˙LX„∞ÑÒ*a’ÉMû5©Ñf¥écd√x˜¬LâÖÜ√Põ}ï	™óè”‹	#¶GMvÌ¬≤[6Ô!D£˘3,î¡«($áNc$
“∞ÄÅ9Ω∞äΩÊ9¿àeùö,mh%ªzéÖ¿–ú≥•a∆◊û◊Û˛E[{£
endstream
endobj
51 0 obj
<< /Filter /FlateDecode /Length 17 >>
stream
xú36¥P0Ä√C. îÏ
endstream
endobj
52 0 obj
<< /Filter /FlateDecode /Length 131 >>
stream
xúEèÀ
!CÔT·Ú>©á’ûÿ˛ØÎ0öAB¯A";Ò0¨ÛÚ6–≈—¢√7˛6’´cï,∫zRVÈêáºÚPi0QƒÖYLCaŒò »ñ2∑·∂MÉ¨lïT≠Év<∂ße´~©maÍ,Ò¬U^∏«
?êK≠wΩUæBS0ó
endstream
endobj
53 0 obj
<< /Filter /FlateDecode /Length 338 >>
stream
xú5R9Æ›@Î}
] ÄvÕúÁ©~ÓﬂÜî_
C¥Väöéïi˘e!U-ì.øÌImâÚ˜…
âíW%⁄•ëP˘<ÖTøgÀºæ÷ú Kï
ììí«%˛óﬁ.Áck?è#w=z`UåÑÀ£kY:ª√öç¸<¶?‚rÆX∑cH
∫q⁄ÔCÛy» fòñä
]Vâ~AÒ†G≠}˜XTX —ÌIpåçPëÄvÅ⁄H9≥ª®/˙Yîò	tÌã"Ó¢¿IÃúb]:˙>t,®ø6„ÀØéJ˙H+kL⁄w£IiÃ"ìÆóEo7o}=∏@Û. ^Õ AS÷(i|–™ùc(öeÖwö4«áÃ<á3îÙ}(~_K&∫(ë?
°_£åúos—ü∂äÒŸaØ`Ö“≈ö‰}@*z`˙ˇ◊¯y˛¸∂ÄT
endstream
endobj
54 0 obj
<< /Filter /FlateDecode /Length 248 >>
stream
xú-Q9íAÀÁzBs”Ô±Àë˜ˇÈ
 ÉÜC :-qP∆Oñ+ﬁÚ»U¥·Ôô¡w¡°ﬂ u9H“TM®]ºΩvfÛ§5,ÉÎ?c
7zqxL∆ŸÌu5{◊kOfP2+q…ƒSuÿ»ô√O¶åÌ\œ
»π÷e§õï∆åÑ#M!RH°Í&©3Aê£´Q£ç≈~ÈÀ#ùaU#j˚\K€◊sŒ4;´<9•GWúÀ…≈+˝ºÕ¿ET´<pø€C˝úÏ‰7ﬁ“π≥≈Ù¯^s≤º0XÒÊµêMµ¯7/‚¯=„Î˘¸®•[
endstream
endobj
55 0 obj
<< /Filter /FlateDecode /Length 72 >>
stream
xú5å±¿0{¶–6X`ÔìKEˆoC|N/ó¢¡Z
∫Ç#pu©¸—#]π)EócŒÇ·q™_H1F=®#„ﬁ«Oπ_p}
endstream
endobj
56 0 obj
<< /Filter /FlateDecode /Length 87 >>
stream
xú5Mπ¿0ÎôÇÃ£ÿÏìKÂÏﬂÏ∏A:} îk‰Ç·ùo!¯¶/ÑuO*ª%:l°Ü≥
íâ·W6xUÆäˆµíâÏl¶1ÿ†e˙—Œ∑Iœ•ﬁò
endstream
endobj
57 0 obj
<< /Filter /FlateDecode /Length 138 >>
stream
xú=èA1ÔyÖ?)vBXﬁ≥UO€ˇ_Kö›^–å1BCo®jõÇ
«ã•K®÷)äâJ»ô`•§“gëzb8‹¥Œ‚±È˙ªíV}–ÊF∫%hÇGÏSi‹ñqƒ5Í)Í\£ºπü©Wÿ4í›¥≤ík8¶ﬂΩÁ©Îˇ”Uﬁ__ﬂ.å
endstream
endobj
58 0 obj
<< /Filter /FlateDecode /Length 210 >>
stream
xú5PÀ
C1ªg
®ÅdûVΩuˇkm–;aˇBX»îy©…Œ)ÈK>:L∂.ø±"≠u%Ï ö û+Ô°ô≤±—ÿ‚`p&^Ä7`Ëiç5t·Ç¶.ïBÅ≈%ô|u{ËæOxjrvC…`	j∫MX¥<üêN‚ˇ~√Ó-‰°íÛ û˘úÌ;≥n·'jv"—r2‘≥4«E<yE¶p‚≥÷w’4‘fNñÆN?å `"^YÄÏÆD9K“é•üoº«˜@ S¥
endstream
endobj
24 0 obj
<< /BaseFont /DejaVuSans /CharProcs 25 0 R
/Encoding <<
/Differences [ 32 /space 40 /parenleft /parenright 44 /comma 46 /period 48 /zero /one
/two /three /four /five /six /seven /eight 61 /equal 77 /M 83 /S 97 /a 99
/c /d /e 103 /g 105 /i 107 /k /l /m /n /o 114 /r 116 /t 118 /v 120 /x /y ]
/Type /Encoding >>
/FirstChar 0 /FontBBox [ -1021 -463 1794 1233 ] /FontDescriptor 23 0 R
/FontMatrix [ 0.001 0 0 0.001 0 0 ] /LastChar 255 /Name /DejaVuSans
/Subtype /Type3 /Type /Font /Widths 22 0 R >>
endobj
23 0 obj
<< /Ascent 929 /CapHeight 0 /Descent -236 /Flags 32
/FontBBox [ -1021 -463 1794 1233 ] /FontName /DejaVuSans /ItalicAngle 0
/MaxWidth 1342 /StemV 0 /Type /FontDescriptor /XHeight 0 >>
endobj
22 0 obj
[ 600 600 600 600 600 600 600 600 600 600 600 600 600 600 600 600 600 600
600 600 600 600 600 600 600 600 600 600 600 600 600 600 318 401 460 838 636
950 780 275 390 390 500 838 318 361 318 337 636 636 636 636 636 636 636 636
636 636 337 337 838 838 838 531 1000 684 686 698 770 632 575 775 752 295
295 656 557 863 748 787 603 787 695 635 611 732 684 989 685 611 685 390 337
390 838 500 500 613 635 550 635 615 352 635 634 278 278 579 278 974 634 612
635 635 411 521 392 634 592 818 592 592 525 636 337 636 838 600 636 600 318
352 518 1000 500 500 500 1342 635 400 1070 600 685 600 600 318 318 518 518
590 500 1000 500 1000 521 400 1023 600 525 611 318 401 636 636 636 636 337
500 500 1000 471 612 838 361 1000 500 500 838 401 401 500 636 636 318 500
401 471 612 969 969 969 531 684 684 684 684 684 684 974 698 632 632 632 632
295 295 295 295 775 748 787 787 787 787 787 838 787 732 732 732 732 611 605
630 613 613 613 613 613 613 982 550 615 615 615 615 278 278 278 278 612 634
612 612 612 612 612 838 612 634 634 634 634 592 635 592 ]
endobj
25 0 obj
<< /M 26 0 R /S 27 0 R /a 28 0 R /c 29 0 R /comma 30 0 R /d 31 0 R
/e 32 0 R /eight 33 0 R /equal 34 0 R /five 35 0 R /four 36 0 R /g 37 0 R
/i 38 0 R /k 39 0 R /l 40 0 R /m 41 0 R /n 42 0 R /o 43 0 R /one 44 0 R
/parenleft 45 0 R /parenright 46 0 R /period 47 0 R /r 48 0 R /seven 49 0 R
/six 50 0 R /space 51 0 R /t 52 0 R /three 53 0 R /two 54 0 R /v 55 0 R
/x 56 0 R /y 57 0 R /zero 58 0 R >>
endobj
3 0 obj
<< /F1 24 0 R /F2 14 0 R >>
endobj
4 0 obj
<< /A1 << /CA 0 /Type /ExtGState /ca 1 >>
/A2 << /CA 1 /Type /ExtGState /ca 1 >>
/A3 << /CA 0.8 /Type /ExtGState /ca 0.8 >> >>
endobj
5 0 obj
<< >>
endobj
6 0 obj
<< >>
endobj
7 0 obj
<< /DejaVuSans-Oblique-sigma 20 0 R /DejaVuSans-Oblique-uni03BC 21 0 R >>
endobj
2 0 obj
<< /Count 1 /Kids [ 10 0 R ] /Type /Pages >>
endobj
59 0 obj
<< /CreationDate (D:20191031162838-05'00')
/Creator (matplotlib 3.1.0, http://matplotlib.org)
/Producer (matplotlib pdf backend 3.1.0) >>
endobj
xref
0 60
0000000000 65535 f 
0000000016 00000 n 
0000023812 00000 n 
0000023496 00000 n 
0000023539 00000 n 
0000023681 00000 n 
0000023702 00000 n 
0000023723 00000 n 
0000000065 00000 n 
0000000385 00000 n 
0000000208 00000 n 
0000009663 00000 n 
0000012141 00000 n 
0000011933 00000 n 
0000011600 00000 n 
0000013194 00000 n 
0000009684 00000 n 
0000010156 00000 n 
0000010315 00000 n 
0000010439 00000 n 
0000010811 00000 n 
0000011163 00000 n 
0000022030 00000 n 
0000021830 00000 n 
0000021319 00000 n 
0000023083 00000 n 
0000013256 00000 n 
0000013415 00000 n 
0000013826 00000 n 
0000014203 00000 n 
0000014506 00000 n 
0000014644 00000 n 
0000014944 00000 n 
0000015262 00000 n 
0000015727 00000 n 
0000015870 00000 n 
0000016190 00000 n 
0000016352 00000 n 
0000016763 00000 n 
0000016903 00000 n 
0000017056 00000 n 
0000017173 00000 n 
0000017501 00000 n 
0000017735 00000 n 
0000018022 00000 n 
0000018174 00000 n 
0000018394 00000 n 
0000018616 00000 n 
0000018737 00000 n 
0000018967 00000 n 
0000019107 00000 n 
0000019497 00000 n 
0000019586 00000 n 
0000019790 00000 n 
0000020201 00000 n 
0000020522 00000 n 
0000020666 00000 n 
0000020825 00000 n 
0000021036 00000 n 
0000023872 00000 n 
trailer
<< /Info 59 0 R /Root 1 0 R /Size 60 >>
startxref
24026
%%EOF

